Dark Sectors 2016 Workshop: Community Report

This report, based on the Dark Sectors workshop at SLAC in April 2016, summarizes the scientific importance of searches for dark sector dark matter and forces at masses beneath the weak-scale, the status of this broad international field, the important milestones motivating future exploration, and promising experimental opportunities to reach these milestones over the next 5-10 years.

==> authorList/README <==
This directory contains tools & data to facilitate creating an author list and author contact email list for the DS2016 workshop.  

CONTACT: Richard van de Water (vdwater@lanl.gov) or Natalia Toro (ntoro@slac.stanford.edu)

**To add an author**
1) Add a row to the spreadsheet MasterAuthorList.csv for the author.  It can be at the end or in alphabetical order.
 - complete every entry in the spreadsheet
 - email address should be just email address with no additional info
 - Institution should be entered following guidelines under "to fix an institution" below.
 - If the person was an editor of the document, then add "editor" to the 5th column to make sure they are not included twice in the author list.
 2) in this directory, run "bash authorScript.bash" to regenerate the email list and authorList2.tex 
 3) verify that the output in emailList.txt and authorList2.tex looks sensible
 4) recompile WorkshopReport.tex in parent directory.

**To fix an institution**
NOTE: Authors with multiple institutions should use slashes, i.e. 
Institution A / Institution B

You have two options for each institution:
__Option A__ 
(recommended if the same institution appears more than once, otherwise optional) 
1) Use an alias starting with backslash (e.g. '\slac') and put that in the spreadsheet in affiliatino column
2) Define that ailas in the file authorAliases.tex
__Option B__
Just enter the full address in the spreadsheet affiliation column BUT please replace all commas with exclamation marks, and avoid using other special characters (& / etc) as these will trip up the TeX compilation.  

Then follow tex compilation steps (2)-(4) above.
